Generalizable Heterogeneous Federated Cross-Correlation and Instance Similarity Learning

Federated learning is an important privacy-preserving multi-party learning paradigm, involving collaborative learning with others and local updating on private data. Model heterogeneity and catastrophic forgetting are two crucial challenges, which greatly limit the applicability and generalizability. This paper presents a novel FCCL+, federated correlation and similarity learning with non-target distillation, facilitating the both intra-domain discriminability and inter-domain generalization. For heterogeneity issue, we leverage irrelevant unlabeled public data for communication between the heterogeneous participants. We construct cross-correlation matrix and align instance similarity distribution on both logits and feature levels, which effectively overcomes the communication barrier and improves the generalizable ability. For catastrophic forgetting in local updating stage, FCCL+ introduces Federated Non Target Distillation, which retains inter-domain knowledge while avoiding the optimization conflict issue, fulling distilling privileged inter-domain information through depicting posterior classes relation. Considering that there is no standard benchmark for evaluating existing heterogeneous federated learning under the same setting, we present a comprehensive benchmark with extensive representative methods under four domain shift scenarios, supporting both heterogeneous and homogeneous federated settings. Empirical results demonstrate the superiority of our method and the efficiency of modules on various scenarios.

==> Version/Old.tex <==
\newcommand{\fedavg}{{FedAVG}}
\newcommand{\fedprox}{{FedProx}}
\newcommand{\fedcurv}{{FedCurv}}
\newcommand{\pfedme}{{pFedME}}
\newcommand{\rcfl}{{RCFL}}
\newcommand{\fccl}{{FCCL}}
\newcommand{\rhfl}{{RHFL}}
\newcommand{\cronus}{{CRONUS}}
\newcommand{\cfd}{{CFD}}
\newcommand{\feddf}{{FedDF}}
\newcommand{\fedmd}{{FedMD}}
\newcommand{\fedkt}{{FedKT}}
\newcommand{\fedgen}{{FEDGEN}}
\newcommand{\fml}{{FML}}
\newcommand{\solo}{{SOLO}}
\newcommand{\lgfedavg}{{LG-FEDAVG}}
\newcommand{\fedmatch}{{FedMatch}}
\newcommand{\moon}{{MOON}}
\newcommand{\furl}{{FURL}}
\newcommand{\oursabbv}{{Ours}}



\newcommand{\FRSL}{Federated Representation Similarity Learning}
\newcommand{\FRSLab}{{FRSL}}
\newcommand{\FCCM}{Federated Cross-Correlation Matrix}
\newcommand{\FCCMab}{{FCCM}}
\newcommand{\FCCSAL}{Federated Cross-Correlation and Representation Similarity Learning}
\newcommand{\FCCSALab}{{FCCSA}}
\newcommand{\FNTD}{Federated Non Target Distillation}
\newcommand{\FNTDab}{{FNTD}}

\newcommand{\digits}{{Digits}}
\newcommand{\officehome}{{Office-Home}}
\newcommand{\officeTO}{{Office31}}
\newcommand{\officecaltech}{{Office Caltech}}
\newcommand{\cifarhun}{{Cifar-100}}
\newcommand{\tyimagenet}{{Tiny-ImageNet}}
\newcommand{\fashionmnist}{{Fashion-MNIST}}

\newcommand{\mnist}{{MNIST}}
\newcommand{\usps}{{USPS}}
\newcommand{\svhn}{{SVHN}}
\newcommand{\syn}{{SYN}}
\newcommand{\art}{{Art}}
\newcommand{\clipart}{{Clipart}}
\newcommand{\product}{{Product}}
\newcommand{\realworld}{{RealWorld}}

\newcommand{\resnet}{{ResNet}}
\newcommand{\efficientnet}{{EfficientNet}}
\newcommand{\mobilenet}{{MobileNet}}
\newcommand{\googlenet}{{GoogLeNet}}

\IEEEraisesectionheading{
\section{Introduction}\label{sec:introduction}}
\IEEEPARstart{C}{urrent} deep neural networks have enabled great success in various computer vision tasks {\cite{ImagenetClassification_NeurIPS12,ResNet_CVPR16,vit_iclr21}}, based on the large-scale and computationally expensive training data {\cite{ImageNet_IJCV15,Cityscapes_CVPR16,COCO_ECCV14,WePerson_MM21}}. However, in real world, data are usually distributed across numerous participants (\eg, mobile devices, organizations, cooperation). Due to the ever-rising privacy concerns and strict legislations {\cite{GDPR17}}, the traditional center training paradigm which requires to aggregate data together, is prohibitive. Driven by such realistic challenges, federated learning {\cite{FLOptimization_arXiv16,FLStrategies_arXiv16,FedAvg_AIST17,Secureml_SP17,FederatedMLConApp_TIST19}} has been popularly explored as it can 
train a global model for different participants rather than centralize any private data. Therefore, it provides an opportunity for privacy-friendly collaborative machine learning paradigm and has shown promising results to facilitate real world applications, such as  keyboard prediction {\cite{FLKeyboard_arXiv18}}, medical analysis{\cite{FLStroke_arXiv20,FedDG_CVPR21}}, person re-identification{\cite{FedReID_MM20}}, and humor recognition {\cite{FLHumorReco_IJCAI2020}}.

Despite the great success afforded by federated learning, there remain fundamental research problems {\cite{Advances_arXiv19,FLChallenges_SPM20}}. 
One common and key challenge  is \textbf{data heterogeneity} {\cite{FLONNonIID_arXiv21}}. In practical, private data distributions of different participants are inherently non-IID (non-independently and identically distributed) since data are usually collected from different sources or scenarios. Existing works {\cite{2PersFL_arXiv21}} have indicated that under heterogeneous data, standard federated learning methods such as FedAvg {\cite{FedAvg_AIST17}} inevitably faces performance degradation or even collapse. A resurgence of methods mainly focus on incorporating extra proximal terms to regularize the local optimization objective close to the global optima in local updating phase {\cite{FedProx_arXiv2018,FedCurv_NeurIPS19,FedDG_CVPR21,MOON_CVPR21,FedProc_arXiv21,FedRS_KDD21}}. However, these methods normally requires noticeably additional computation cost or dedicated hyper parameters  to obtain promising performance, which increases the burden for participants and is not suitable for large-scale scenarios. Besides, most of them tackle the data in label skew {\cite{FLonNONIDD_NC21}}, where the label distribution of different participants is inconsistent, but ignore the fact that there exists \textbf{domain skew}. In detail, feature distribution of participants private data may be strikingly different {\cite{DatasetShiftML_2009,SurveyonTF_TKDE09,UniViewonDatasetShift_PR12}} in complex  environment. Thus, private model would suffer from drastic performance drop on others domains with disparate feature distribution. As a result, forcing private model to acquire generalizable ability under domain skew would be important and meaningful. 
The other inescapable and practical challenge is \textbf{model heterogeneity}. Specifically, participants have the  option of architecting private models rather than agreeing on the pre-defined architecture, because they may have different design criteria, distinctive hardware capability {\cite{Fbnet_CVPR19,Fednas_arXiv20}}  or intellectual property rights {\cite{IPR_06}}. Thus, taking into account data heterogeneity and model heterogeneity together, previously aforementioned methods are no longer feasible because they are based on sharing consistent model architecture for parameter averaging operation. In order to address this problem, existing efforts can be taxonomized into two major categories: shared global model {\cite{FML_arXiv20,FLwiMoE_2020,LGFEDAVG_NeurIPS20}} and knowledge transfer {\cite{FedMD_NeurIPS19,Cronus_arXiv19,FedMDNFDP_arXiv20,FedDF_NeurIPS20,FedGKT_NeurIPS20,DeFLMKT_IoTJ21,RoFL_CVPR22}}. However, leveraging extra global model not only raises the communication cost but also necessitates additional model structure in participant side. For knowledge transfer methods, provided with unlabeled public data or artificially generated data, they utilize knowledge distillation {\cite{ModelComp_KDD06,KnowDistilling_arXiv15}} to transfer the logits output on public data among participants. However, this strategy is subject to a significant limitation: they conduct knowledge transfer via logits distillation, which is in high semantic level {\cite{DKD_CVPR22}} and thus directly align distribution probably provides wrong optimization direction {{\cite{DetectOOD_NeurIPS18,ConfinEsit_CVPR20}}} since the category of public data is unknowable and is highly possible in semantic inconsistent with private data.
Thus, considering data and model heterogeneity together, an essential issue has long been overlooked: \textsl{(a) How to achieve better generalizable ability in heterogeneous federated learning?}

Besides, compared to label skew, in domain skew, data are typically from various domains rather same domains. Private models are required to present satisfactory performance on not only intra domain but also others domains. However, a major hindrance is from federated learning paradigm. In general, federated learning could be regarded as a cyclic process with two steps: collaborative updating and local updating {\cite{FedAvg_AIST17,FederatedMLConApp_TIST19}}. In collaborative updating, participants learn from others. In local updating, model is solely trained on private data, which is prone to overfit current knowledge and forgets previously learned knowledge, resulting in \textbf{catastrophic forgetting} {\cite{CataInter_PLM89,Connectionist_PR90,Catastrophic_99,EmpInvCataFor_arXiv13}}. Existing related methods mainly focus on introducing parameter stiffness to regulate learning objective  {\cite{FedProx_arXiv2018,FedCurv_NeurIPS19,pFedME_NeurIPS20,MOON_CVPR21,RoFL_CVPR22}}, which either rely on model homogeneity or do not take full advantage of the underlying inter domain knowledge provided from models which are optimized in collaborative learning. Consequently, a natural question arises: \textsl{(b) How to effectively balance multiple domains knowledge to avoid catastrophic forgetting?} An illustration of these two problems in shown in Figure.

To acquire generalization ability in heterogeneous federated learning, inspired by self-supervised learning with information maximization{\cite{W-MSE_NeurIPS20,Barlow_ICML21,vicreg_ICLR22}}, a preliminary version of this work published in CVPR 2022 \cite{FCCL_CVPR22} explores \textbf{\FCCM} (\FCCMab). In particular, we aim to makes same dimensions of logits output highly correlated to learn class invariance and decorrelate pairs of different dimensions within logits output to stimulate the diversity of different classes. Moreover, representation  (embedding feature) exhibits generic information related to structural information {\cite{CRD_ICLR20}}, but is a lack of effective utilization. This motivates us to capture significantly more information in other participants models representation. We propose \textbf{\FRSL} (\FRSLab), which leverage unlabeled public data to innovatively align instance similarity distribution among participants. Specifically, for each unlabeled public sample, private network calculates feature output and obtains its similarity with respect to others in the batch. We convert the individual feature distribution into similarity probability distribution. Then, we transfer that knowledge, so that participants are required to mimic the same similarity distribution. This approach offers a practical solution for differential feature shape in model heterogeneous federated learning. Besides, we assume that \FCCMab{} is essential because optimizing classifier in collaborative learning is beneficial to alleviate its bias to local data distribution {\cite{ClassCal_NeurIPS21,FedUFO_ICCV21}}. 
To this end, we develop \textbf{\FCCSAL} (\FCCSALab) in heterogeneous federated learning, which not only handles the communication problem but also lean a more generalizable representation in heterogeneous federated learning.

To better preserve inter domain knowledge, we propose to use distillation to extract useful knowledge from respective previous model which captures the inter domain knowledge after communicating with other participants. Compared to popular knowledge distillation strategy {\cite{KnowDistilling_arXiv15,BornAgainKD_ICML18,TeaAsskD_AAAI20,PSKD_CVPR21}}, we disentangle the logits output into target and non-target distillation {\cite{BornAgainKD_ICML18,KR_AAAI21,DKD_CVPR22}}. We conjecture that target distillation concentrates on the intra domain knowledge since it represents the supervision of target class, which is related to intra domain knowledge and previous model could not precisely infer, resulting in optimization conflict.  
But non-target distillation depicts the posterior probability of similarities among classes provided by previous model which contains privileged information of inter domain, and hence ensure generalization ability {\cite{RNNwtKD_ICASSP16,UnifDis_ICLR16,DoesKDWork_NeurIPS21}}. 
Therefore, we propose \textbf{\FNTD} (\FNTDab) to better transfer inter domain knowledge from previous model, which alleviates catastrophic forgetting and does not incur much extra computation, reaching both effective and flexible knowledge transfer in local updating phase. In addition, for intra domain knowledge forgetting problem, we intuitively leverage label information to constrain optimization direction such as (\ie, CrossEntropy {\cite{CE_AOR05}}). 


This paper build upon on our conference paper \cite{FCCL_CVPR22}. However, this paper extends our earlier work in several important aspects:

\begin{itemize} 
	\item We introduce a novel and effective knowledge transfer strategy, \FRSLab{} in heterogeneous federated learning. Through measuring and aligning the similarity distribution among unlabeled public data, heterogeneous models realize feature-level knowledge communication which learns more information from others and hence acquires better generalizable ability.
	
	\item We disentangle the traditional knowledge distillation and develop \FNTDab{} to better preserve inter domain knowledge. Cooperated with simple intra domain constraint, it effectively balances multiple domains knowledge and avoids knowledge catastrophic forgetting.  
	
	\item We rigorously validate proposed method on massive experiments (\ie, \digits{} {\cite{MNIST_IEEE98,USPS_TPAMI94,svhn_NeurIPS11,syn_arXiv18}}, \officecaltech{} {\cite{OffCaltech_CVPR12}}, \officeTO{} {\cite{office31_ECCV10}} and \officehome{} {\cite{officehome_CVPR17}})) with unlabeled public data (\ie, \cifarhun{} \cite{cifar_Toronto}, \tyimagenet{} \cite{ImageNet_IJCV15}). We further provide detailed ablation studies and in-depth discussions to validate its efficacy and robustness.
% 	\item We conduct extensive experiments on two image classification tasks (\eg, \digits {\cite{MNIST_IEEE98,USPS_TPAMI94,svhn_NeurIPS11,syn_arXiv18}} and \officehome {\cite{officehome_CVPR17}}) with unlabeled public data {\cite{cifar_Toronto,ImageNet_IJCV15,fashionmnist_arXiv17}}. \ourabbrv{} achieves superior inter and intra domain performance over related methods. Ablation study on core module validates its efficacy and indispensability.
\end{itemize}

% A preliminary version of this work has been published in CVPR 2022 \cite{FCCL_CVPR22}. This paper has the following improvements. 
% First, we provide an effective and feasible solution for differential feature learning to achieve better generalizable performance.
% Second, we design a powerful and simple non-target distillation strategy to fully utilize the inter domain knowledge. 
% To demonstrate its effectiveness, we provide a comprehensive evaluation of existing state-of-the-art methods. The experiments show that our simple yet powerful baseline achieves surprising advantage. Last but not least, we validate the superiority of the proposed methods through extensive experiments, together with detailed ablation studies and in-depth discussions. We believe it will serve as a fundamental operation to boost performance.

% In this work, we propose a a simple yet strong method for heterogeneous federated learning. In fact, the proposed distillation modules can be implemented by a few lines of code. Despite its simplicity, experiments demonstrate the effectiveness of our method. The overview of our method is illustrated in Fig. 2. In a nutshell, 

% Our main contributions are summarized below:


\section{Related Work}\label{sec:related}


\subsection{Heterogeneous Federated Learning}



\noindent \textbf{Data Heterogeneity}. A pioneering work proposed the currently most widely used algorithm, \fedavg {\cite{FedAvg_AIST17}}. But it suffers  performance deterioration on non-i.i.d data (data heterogeneity). Shortly after, a large body methods {\cite{FedProx_arXiv2018,FedCurv_NeurIPS19,pFedME_NeurIPS20,MOON_CVPR21,RoFL_CVPR22,ClassCal_NeurIPS21}} research on non-IID data. These methods mainly focus on label skew  with limited domain skew. However, when private data sampled from different data domains, these works do not consider inter domain performance but only focus on learning an internal model. Latest researches have studied related problems of unsupervised domain adaptation for target domain {\cite{FADA_ICLR20,fMRIAna_MIA20}} and domain generalization on unseen domains {\cite{FedDG_CVPR21}}. However, collecting data in the target domain can be time-consuming and impractical. Meanwhile, considering the performance on unknown domains is an idealistic setting. For more realistic settings, participants are probably more interested in the performance on other domains, which could directly improve economic benefits. In this work, we focus on improving inter domain performance under domain skew.

\noindent \textbf{Model Heterogeneity}.
With the demand for unique models, federated learning with model heterogeneity has been an active area of research. One Direction is introducing shared extra model such as \fml {\cite{FML_arXiv20}} and \lgfedavg {\cite{LGFEDAVG_NeurIPS20}}. However, these techniques may not be applicable when considering the additional computing overhead and expensive communication cost. \fedmd {\cite{FedMD_NeurIPS19}}, \cronus {\cite{Cronus_arXiv19}} and \cfd {\cite{CFD_arXiv20}} operate on labeled public data (with similar distribution) via knowledge distillation {\cite{ModelComp_KDD06,KnowDistilling_arXiv15}}. Therefore, these approaches heavily rely on the quality of labeled public data, which may not always be available on the server. Latest works (\eg, \feddf {\cite{FedDF_NeurIPS20}}, \fedkt {\cite{FedKT_arXiv20}} and \fedgen {\cite{FEDGEN_ICML21}}) have proven the feasibility to do distillation on unlabeled public data or synthetic data. However, these methods leverage unlabeled public data to reach semantic information consistency, which are not suitable to learn a generalizable representation and and thus lead to a sub-optimal inter domain performance. In this paper, based on unlabeled public data, we construct correlation matrix and measure representation similarity on unlabeled public data to reach generalizable ability.


\subsection{Catastrophic Forgetting}
Catastrophic forgetting {\cite{CataInter_PLM89,Connectionist_PR90,Catastrophic_99,EmpInvCataFor_arXiv13}} has been an essential problem in incremental learning {\cite{silver2002task,ExpertGate_cvpr17,MAS_eccv18}} when models continuously learn from a stream data, with the goal of gradually extending acquired knowledge and using it for future learning {\cite{CataInter_PLM89,EmpInvCataFor_arXiv13}}.  Existing incremental learning works on tackling catastrophic forgetting can be broadly divided into three branches {\cite{AConLearSurvey_TPAMI21}}: replay methods {\cite{iCARL_CVPR17,DGR_NeurIPS17,e2eil_ECCV18,GenReplay_arXiv18,ER_ICLR19,Unified_CVPR19,Dark_NeurIPS20,COIL_MM21,SCR_CVPR21}}, regularization-based methods {\cite{EWC_PNAS17,LwF_TPAMI17,MAS_eccv18,NullSpace_CVPR21,PASS_CVPR21,calibrateCIL_ICME21,IL2A_NeurIPS21}} and parameter isolation methods {\cite{Pathnet_arXiv17,Packnet_CVPR2018,Piggyback_CVPR18,Nettailor_CVPR19,CPG_NeurIPS19,IADM_SIGKDD19,PNN_arXiv16,ExpertGate_cvpr17,RbkR_CVPR21,DER_CVPR21,DyTox_arXiv21}}. As for federated learning, data are distributed rather than sequential like incremental learning. Despite these differences, both incremental learning and federated learning share a common challenge - how to balance the knowledge from different data distribution.  
Unlike incremental learning methods, we focus on alleviate catastrophic forgetting in distributed data rather than time series data. In particular, we expect to balance and boost both inter and intra domain performance in local updating phase.


\subsection{Self-Supervised Learning}
Self-supervised Learning has emerged as a powerful method for learning useful representation without supervision from labels. Many related methods are based on contrastive methods {\cite{instdisc_cvpr18,IISF_CVPR19,AIISMang_PAMI20,SSLPreInvar_CVPR20,CMC_ECCV20,MOCO_CVPR20,SimCLR_ICML20,ISD_ICCV21}}. This kind method contrasts positive pairs against negative pairs, where positive pairs are often formed by same samples with different data augmentations and negative pairs are normally other different samples. Recently, another line of works {\cite{BYOL_NeurIPS20,SimSiam_CVPR21}} employs asymmetry of the learning update (stop-gradient operation) to avoid trivial solutions. Besides, a principle to prevent collapse is to maximize the information content of the embeddings {\cite{W-MSE_NeurIPS20,Barlow_ICML21,vicreg_ICLR22}}.
The key difference between \FCCMab{} and above method is that aforementioned efforts rely on siamese networks to apply weight-sharing or momentum-updating strategies. Therefore, leveraging unlabeled public data to directly construct self-supervised learning paradigm is not feasible for model heterogeneous federated learning because models are in distinct architecture.




\subsection{Knowledge Distillation}
Knowledge distillation aims to transfer knowledge from one network to the other  {\cite{ModelComp_KDD06,KnowDistilling_arXiv15}}. The knowledge from the teacher network can be extracted and transferred in various ways and can be mainly divided into three directions: logits distillation {\cite{KnowDistilling_arXiv15,RNNwtKD_ICASSP16,UnifDis_ICLR16,BornAgainKD_ICML18,TeaAsskD_AAAI20,PSKD_CVPR21,KR_AAAI21,DKD_CVPR22}}, feature distillation {\cite{Fitnets_ICLR15,OverFeaDis_ICCV19,CRD_ICLR20,SemCKD_AAAI21}} and relation distillation {\cite{GiftKD_CVPR17,SP_CVPR19,RKD_CVPR19,CCKD_CVPR19}}. In this work , we propose \FRSLab{} to implement multi-party rather than pair-wise heterogeneous feature communication in collaborative updating. Furthermore, we investigate how to better maintain the inter domain knowledge in local updating. Thus, we develop \FNTD{} to disentangle typical logits distillation, which assures the inter domain performance without heavy computational strain.


\section{Methodology}\label{sec:Methodology}
\textbf{Problem Statement and Notations.}
Following the standard federated learning setup, there are $K$ participants (indexed by $i$). The $i^{th}$ participant has a local model $\theta_i$ and private data $D_i =\{(X_i,Y_i)|X_i \in \mathbb{R}^{N_i \times O}, Y_i \in \mathbb{R}^{N_i \times C}\}$, where $N_i$ denotes the scale of private data, $O$ represents input size and $C$ is defined as the number of classes for classification. We further consider local model with two components: feature extractor and unified classifier. The feature extractor $f \, : \mathcal{X} \rightarrow \mathcal{H}$, maps input image $x$ into a compact $d$ dimensional feature vector $h = f(x) \in \mathbb{R}^d$. A unified classifier $g: \mathcal{Z} \rightarrow \mathbb{R}^{C}$, produces probability output, $g(h)$ as prediction for $x$.  Thus, the overall private model is denoted as $\theta_i=(f_i,g_i)$ Furthermore, in heterogeneous federated learning, \textbf{data heterogeneity} and \textbf{model heterogeneity} are defined as following:

\begin{itemize}
\item \textbf{Data heterogeneity}: $P_i(X|Y)\neq P_j(X|Y)$. There exists domain skew among private data, \ie, conditional distribution $P(X|Y)$ of private data vary across participants even if $P(Y)$ is shared. Specifically, same label $Y$ has distinctive feature $X$ in different domains. 

\item \textbf{Model heterogeneity}: $Shape(\theta_i) \neq Shape(\theta_j)$. Participants architect models independently, \ie, for classification tasi, the selected feature extractor $f$ are different such as \resnet {\cite{ResNet_CVPR16}, \efficientnet {\cite{EfficientNet_ICML19}}} and \mobilenet {\cite{Mobilenets_arXiv17}}, and hence the   classifier module is also differential.
\end{itemize}

The unlabeled public data $D_0 = \{X_0|X_0 \in \mathbb{R}^{N_0 \times D}\}$ is adopted to  achieve heterogeneous models  communication, which is relatively easy to access in real scenarios, \eg, existing datasets{ \cite{COCO_ECCV14,ImageNet_IJCV15,Cityscapes_CVPR16,WePerson_MM21}} and web images{\cite{Webvision_arXiv17}}. 
The goal for $i^{th}$ participant is to reach communication and learn a model $\theta_i$ with generalizable ability. Besides, considering \textbf{catastrophic forgetting}, the optimization objective for $\theta_i$ is to present both higher and stabler inter and intra domain performance.

\subsection{\FCCM}\label{sec:3.1}
\textbf{Motivation of Dimension-Level Operation}.
Motivated by {information maximization} {\cite{Infobot_arXiv2000,Barlow_ICML21,vicreg_ICLR22}}, a generalizable representation should be as informative as possible about image, while being as invariant as possible to the specific domain distortions that are applied to this sample. In our work, domain skew leads distinctive feature $X$ for the same label $Y$ in different domains. 
Therefore, the distribution of logits output along the batch dimension on different domains is not identical.
Moreover, different dimensions of logits output are corresponding to distinct classes. 
Thus, we need to encourage the invariance of same dimensions and the diversity of different dimensions.
Private data carries specific domain information and is under privacy protection, which is not suitable and feasible to conduct contrastive learning. Therefore, we leverage the unlabeled public data, which are normally generated and collected from multi domains. We optimize private models through requiring logits output invariant to domain distortion and decorrelating different dimensions of logits output on unlabeled public data.

\noindent \textbf{Construct Federated Cross-Correlation Matrix}.
Specifically, we obtain the logits output from $i^{th}$ participant: $Z_i=g(f(X_0)) \in \mathbb{R}^{N_0 \times C}$. For $i^{th}$ and $j^{th}$ participant, the logits output on 
unlabeled public data is $Z_i$ and $Z_j$. 
Notably, considering the computing burden on the server side, we calculate average logits output: $\overline{Z}=\frac{1}{K}\sum_iZ_i$. Then, we calculate  cross-correlation matrix, $\mathcal{M}_i$ for $i^{th}$ participant with average logits output as:

\begin{equation}
\mathcal{M}_i^{uv} \triangleq \frac{
\sum_b ||Z_i^{b,u}|| ~~ ||\overline{Z}^{b,v}||}
{\sqrt{\sum_b {||Z_i^{b,u}||}^2} \sqrt{\sum_b {||\overline{Z}^{b,v}||}^2}}.
\label{eq:avgcrosscorr}
\end{equation}
The $b$ indexes batch samples,  $u,v$ index the  dimension of logits output and $||\  ||$ is the normalization operation along the batch dimension. $\mathcal{M}_i$ is a square matrix with size of output dimensionality, $C$ and values comprised between -1 (\ie, dissimilarity) and 1 (\ie, similarity). 
Then, the \FCCMab{} loss for $i^{th}$ participant is defined as:

\begin{equation}
\mathcal{L}_{{\FCCMab}} =  {\sum_u  (1-\mathcal{M}_i^{uu})^2} + \lambda {\sum_{u}\sum_{v \neq u} {(1+\mathcal{M}_i^{uv}})^2},
\label{eq:fccl_loss}
\end{equation}
where $\lambda$ is a positive constant trading off the importance of the first and second terms of  loss. Naturally, when on-diagonal terms of the  cross-correlation matrix take the value $+1$, it encourages the logits output from different participants to be similar; when off-diagonal terms of the  cross-correlation matrix take value $-1$, it encourages the diversity of logits output, since different dimensions of these logits output will be uncorrelated to each other.

\noindent \textbf{Comparison with Analogous Methods}. 
\fedmd{} \cite{FedMD_NeurIPS19} is based on minimizing mean square error on relative public data with annotation. \feddf{} \cite{FedDF_NeurIPS20} reaches logits output distribution consistency on unlabeled public data.  However, \FCCMab{} expects to achieve correlation of same dimensions but decorrelation of different dimensions on unlabeled public data. Besides, we do operation along the batch dimension, which means that we view unlabeled public data as ensemble rather than individual sample. It is advantageous to eliminate anomalous sample disturbance. We further illustrate the conceptual comparison between \FCCMab{} and \feddf{} in \cref{fig:ConceptCompar}.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\linewidth]{Figure/Core_Comp/diff_fccl.pdf}
		\put(-17.5,6.5){\small{\cite{FedDF_NeurIPS20}}}
	\end{center}
    \caption{\textbf{Conceptual comparison.} The unlabeled public data $D_0(X_0)$ with batch size $B_0$ and input size $O$ are fed into different models. The logits output $Z_i=g_i(f_i(X_0))$ has $C$ dimensions. (a) \FCCMab{} learns invariance in same dimensions and decorrelates pairs of different dimensions on the batch-wise normalized logits output in \cref{eq:avgcrosscorr}. (b) \feddf {\cite{FedDF_NeurIPS20}} calculates the distribution divergence where instance-wise normalized logits output is compared inside a batch. See \cref{sec:3.1} for details.}
	\label{fig:ConceptCompar}
\end{figure}


\definecolor{azure}{rgb}{0.0, 0.5, 1.0}

\begin{algorithm}[t]
\SetNoFillComment
\SetArgSty{textnormal}
\small{\KwIn{Communication epochs $E$, local rounds $T$, participants number $K$, unlabeled public data $D_0(X_0)$, $i^{th}$ private data $D_i(X_i,Y_i)$ , hyper-parameter $\lambda, \mu, \omega,\tau$}}
\BlankLine

% lamda 是 FCCM的那个0.0051 参数
% \mu 是相似度分布的参数

% \tau 是local updating的温度
\For {$e=1, 2, ..., E$}{
    
    \For {$i=1, 2, ..., K$}{
    $H_i = f_i^e(X_0)$  \tcp*{feature vector} 
    $Z_i = g_i^e(H_i)$ \tcp*{logits output}
    $S_i \leftarrow (H_i,\mu)$ by \cref{eq:simmat_old} and \cref{eq:simmat_new} \tcp*{similarity distribution}
    }
    
    $\overline{S} = \frac{1}{K}\sum_iS_i$ \\
    $\overline{Z} = \frac{1}{K}\sum_iZ_i$
    
    \For {$i=1, 2, ..., K$ \textbf{in parallel}}{
    % \tcp{ \scriptsize{Learn Generalizable Representation}}
    
    $\mathcal{L}_{{\FCCMab{}}} \leftarrow$ \textbf{{\FCCM{}}}~($Z_i$, $\overline{Z}$)  
    
    $\mathcal{L}_{{\FRSLab{}}} \leftarrow$ \textbf{{\FRSL{}}}~($S_i$, $\overline{S}$)
    
    $\mathcal{L}_{COL} =\mathcal{L}_{{\FCCMab{}}} + \omega * \mathcal{L}_{{\FRSLab{}}}$
    
    $\theta_i^e \leftarrow \theta_i^e - \eta \mathcal{L}_{COL}$
    
    $\theta_i^{e+1} \leftarrow $ \textbf{\FNTD{}} ($\theta_i^{e-1}$, $D_i$)
    }
}
return $\theta_i^{E+1}$

\BlankLine
\textbf{\FCCM}~($Z_i$, $\overline{Z}$)  

{\color{azure}{See Detail in \cref{sec:3.1}}} 

    $\mathcal{M}_i \leftarrow (Z_i,\overline{Z})$ { by \cref{eq:avgcrosscorr}}
    
     $\mathcal{L}_{\FCCMab{}} \leftarrow (\mathcal{M}_i,\lambda)$ through \cref{eq:fccl_loss} 
     
return $\mathcal{L}_{\FCCMab{}}$

\BlankLine
\textbf{\FRSL{}}~($S_i$, $\overline{S}$)  

{\color{azure}{See Detail in \cref{sec:3.2}}} 

     $\mathcal{L}_{\FRSLab{}} \leftarrow (S_i)$ via \cref{eq:simkd} 
     
return $\mathcal{L}_{\FRSLab{}}$


\textbf{\FNTD}~($\theta_i^{t-1}$, $D_i$): 

{\color{azure}{See Detail in \cref{sec:3.3}}} 


\For{$t = 1, 2, ..., T$}{
    % \For{each batch $\textbf{b} = \{x, y\}$ of $^i$}{

        
        $Z_{i}^{e}=g_i^e(f_i^{e}(X_i))$

        
        $\mathcal{L}_{CE} \leftarrow \texttt{CE}(Y_i, Z_{i}^e)$ in \cref{eq:localCE}
        
        $Z_{i}^{e-1}=g_i^{e-1}(f_i^{e-1}(X_i))$


        $\mathcal{L}_{\FNTDab{}} \leftarrow (Z_i^{e-1}, Z_i^{e}, \tau)$ by \cref{eq:fntd}
        
        $\mathcal{L}_{LOC} = \mathcal{L}_{CE}+\mathcal{L}_{\FNTDab{}}$
        
        $\theta_i^{e} \leftarrow \theta_i^{e}-\eta \nabla \mathcal{L}_{LOC}$
        
}

$\theta_i^{e+1} \leftarrow \theta_i^{e}$

return $\theta_i^{e+1}$ 
\caption{The Proposed Method}
\label{alg:ours}
\end{algorithm}

\subsection{\FRSL}\label{sec:3.2}
\noindent \textbf{Feature-Level Communication Dilemma}.
It is known that embedding feature can be convenient to express
many generic priors about the world {\cite{RepreSurvey_PAMI13,CRD_ICLR20}}, \ie, priors that are not task specific but would be likely to be useful for generalization ability. Intuitively, it is beneficial to conduct feature-level communication in federated learning. However, in model heterogeneous federated learning, embedding features are in distinctive structure for different participants. 

\noindent \textbf{Representation Similarity Alignment}.
Due to the heterogeneous feature, we formulate a novel and simple approach for the feature-wise communication on the basis of instance similarity distribution on unlabeled public data. Formally, Given  $B_0$ a batch of unlabeled public data $D_0$, the $i^{th}$ private model $\theta_i$  maps  them into embedding feature vectors $H_i = f(B_0) \in \mathbb{R}^{|B_0|\times d}$. Let $S_i$ represents the similarity distribution of feature vector among unlabeled public data batch computed by the $i^{th}$ private model and is defined as:

\begin{equation}
\begin{split}
S_i \triangleq ||H_i||_2 \cdot ||H_i||_2^T/\mu \in \mathbb{R}^{|B_0|\times |B_0|},
\label{eq:simmat_old}
\end{split}
\end{equation}
where $|| \ ||_2$ represents $\ell_2$ normalization, $\mu$ is the temperature parameter, $(\ )^T$ means transpose operation and $(,\cdot,)$ represents inner product. Note that, we eliminate the diagonal value in the $S_i$, which is the similarity distribution with itself and poses large value, resulting in dominant effect for the whole similarity distribution. Hence, the $S_i$ is rewritten into:
\begin{equation}
\begin{split}
S_i = S_i \odot \left[ \begin{array}{cccc}
0 & 1 & \cdots& 1 \\
1 & 0 & \cdots  & 1 \\
\vdots & \vdots & \ddots & 1 \\
1 & 1 & 1  & 0
\end{array} 
\right ] \in \mathbb{R}^{(|B_0|-1) \times (|B_0|-1)}.
\label{eq:simmat_new}
\end{split}
\end{equation}
Similarly, it is important to control the server-side computing overhead, so we calculate the average similarity distribution: $\overline{S}=\frac{1}{K}\sum_iS_i$.  Finally, the \FRSL{} (\FRSLab{}) optimization objective  for $i^{th}$ participant is:

\begin{equation} 
\mathcal{L}_{\FRSLab{}}=\sigma(\overline{S})\log \frac{\sigma(\overline{S})}{\sigma(S_i)},
\label{eq:simkd}
\end{equation}

where $\sigma$ denote \texttt{softmax} function. As shown in \cref{eq:simkd}, We achieve the purpose that feature-level communication in model heterogeneous federated learning leans more versatile information from others and results in more generalizable ability. We further illustrate \FRSLab{} in \cref{fig:Illu_FCSL}.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\linewidth]{Figure/Core_Comp/vis_fcsl.pdf}
	\end{center}
    \caption{\textbf{Illustration of \FRSLab{}}. The private model maps unlabeled public data into embedding feature vector $H_i = f_i(X_0)$. We calculate similarity distribution $S_i$ by \cref{eq:simmat_old} and \cref{eq:simmat_new}. Then, optimize present model to align it via \cref{eq:simkd}. See \cref{sec:3.2} for details.}
	\label{fig:Illu_FCSL}
\end{figure}


\noindent \textbf{Overall Objective in Collaborative Updating}.
By combining $\mathcal{L}_{\FCCMab{}}$ in (\ref{eq:fccl_loss}) and $\mathcal{L}_{\FRSLab{}}$ in (\ref{eq:simkd}), the overall loss in collaborative updating becomes:
\begin{equation} 
\mathcal{L}_{COL} = \mathcal{L}_{\FCCMab{}}+\omega * \mathcal{L}_{\FRSLab{}}.
\label{eq:col_loss}
\end{equation}


\subsection{\FNTD}
\label{sec:3.3}
\textbf{Typical Knowledge Distillation}.
Leveraging previous model optimized in collaborative learning to conduct knowledge distillation is useful to regulate that the ongoing model behavior should not deviate too much from it. It is beneficial to maintain inter domain knowledge and mitigate catastrophic forgetting. Existing methods mainly follow three lines: feature distillation, relation distillation and logits distillation {\cite{KDSurvey_IJCV_21}}. However, compared with collaborative updating phase where major computational cost is allocated to server rather participants, in local updating phase, private models are required to train for multiple epochs and the first two distillation methods pose markedly larger computational cost than logits distillation. Thus, leveraging logits knowledge distillation is feasible and practical in local updating. We denote $\mathcal{T}$ and $\mathcal{S}$  as the teacher and the student models, respectively. The logits distillation loss is defined as:

\begin{equation}
    \begin{split}
    \mathcal{L}_{{KD}}&= \text{KL}(\mathbf{p}_{\mathcal{T}}|| \mathbf{p}_{\mathcal{S}}) 
    = \sum_{u}^{C} p_{\mathcal{T}}^{u}\log(\frac{p_{\mathcal{T}}^{u}}{p_{\mathcal{S}}^{u}})\\
    \end{split}
    \label{eq:kd_ork_form}
\end{equation}


 
\begin{equation}
\begin{split}
{\mathbf{p}(x,\theta)} &=[{p}^{1}, .., {p}^{t}, .., {p}^{C}] \in \mathbb{R}^{1\times C} \\
    p^{u}(x,\theta) &= \frac{\exp(z^{u} / \tau)}{\sum_{v}^{C} \exp(z^{v} / \tau)}, z = g(f(x))
\end{split}
    \label{defpi}
\end{equation}
where  $z^u$ represents the logits output of $u^{th}$ class and $\tau$ is temperature hyper-parameter. 
Besides, in local updating, leveraging private data label information to construct CrossEntropy {\cite{CE_AOR05}} loss is helpful to maintain intra domain knowledge {\cite{FedBN_ICLR21,FedMD_NeurIPS19,FedDF_NeurIPS20,FedDF_NeurIPS20}}: 
\begin{equation} 
\mathcal{L}_{CE}=-\bm{1}_{y}\log(\mathbf{p})=-\sum_{u}^C y^u\log(p^u).
\label{eq:localCE}
\end{equation}
We carry out the following optimization objective for $k^{th}$ participant in local updating:


\begin{equation}
    % \mathcal{L}_{\text{LOC}}(D_k,\theta_{\mathcal{T}}) = \mathcal{L}_{\text{CE}}(X_k,Y_k)+
    % \mathcal{L}_{\text{KD}}(X_k,{\theta_{\mathcal{T}}}).
    \mathcal{L}_{{LOC}} = \mathcal{L}_{{CE}}+
    \mathcal{L}_{{KD}}.
    \label{eq:orilocalobj}
\end{equation}
Here $\theta_\mathcal{S}$ is the ongoing model and $\theta_\mathcal{T}$ is previously learned model as teacher model in knowledge distillation. Such training objective design mainly suffers from two limitations. \textbf{1)} Motivated by {\cite{DKD_CVPR22}}, the logits distillation formulation in \cref{eq:kd_ork_form} can be rewritten as:

\begin{equation}
	\begin{split}
	\mathcal{L}_\text{KD} &= p_{\mathcal{T}}^{t}\log(\frac{p_{\mathcal{T}}^{t}}{p_{\mathcal{S}}^{t}}) + p_{\mathcal{T}}^{\backslash t}\sum_{u\neq t}^{C} \hat p_{\mathcal{T}}^{u}(\log(\frac{\hat p_{\mathcal{T}}^{u}}{\hat p_{\mathcal{S}}^{u}}) +\log(\frac{p_{\mathcal{T}}^{\backslash t}}{p_{\mathcal{S}}^{\backslash t}})) \\
	&= \underbrace{p_{\mathcal{T}}^{t}\log(\frac{p_{\mathcal{T}}^{t}}{p_{\mathcal{S}}^{t}}) + p_{\mathcal{T}}^{\backslash t} \log(\frac{p_{\mathcal{T}}^{\backslash t}}{p_{\mathcal{S}}^{\backslash t}})}_{{\text{KL}(\mathbf{b}_{\mathcal{T}}||\mathbf{b}_{\mathcal{S}})}} + p_{\mathcal{T}}^{\backslash t} \underbrace{\sum_{u\neq t}^{C} \hat p_{\mathcal{T}}^{u} \log(\frac{\hat p_{\mathcal{T}}^{u}}{\hat p_{\mathcal{S}}^{u}})}_{\text{KL}(\hat{\mathbf{p}}_{\mathcal{T}} || \hat{\mathbf{p}}_{\mathcal{S}})},\\
	\end{split}
	\label{eq:dkd}
\end{equation}

\begin{equation}
	\begin{split}
	\mathcal{L}_\text{KD} &= \text{KL}(\mathbf{b}_{\mathcal{T}}||\mathbf{b}_{\mathcal{S}}) + p^{\backslash t}_{\mathcal{T}}  \text{KL}(\hat{\mathbf{p}}_{\mathcal{T}} || \hat{\mathbf{p}}_{\mathcal{S}})	\\
    \mathbf{b} & =[p^t, p^{\backslash t}=1-p^t] \in \mathbb{R}^{1\times 2}\\
    \hat{\mathbf{p}} &=[\hat{p}^{1}, .., \hat{p}^{t-1}, \hat{p}^{t+1}, .., \hat{p}^{C}] \in \mathbb{R}^{1\times (C-1)}\\
    \hat{p}^{u} &= \frac{\exp(z^{u} / \tau)}{\sum_{v\neq t}^{C} \exp(z^{v} / \tau)}
    \end{split}
	\label{eq:dkdnotation}
\end{equation}

In the above, the second term of \cref{eq:dkd} could be viewed as the similarity distribution on non target categories and we argue that it includes the privileged information of inter domain which is helpful for alleviating catastrophic forgetting {\cite{PriviInfo_JMLR15,UnifDis_ICLR16}}. However it is negative correlation with  teacher model confidence, $p^{t}_{\mathcal{T}}$ on the target class $t$, which highly suppress the inter domain knowledge transfer. \textbf{2)} Furthermore, there exists optimization direction conflict. Specifically, the gradient 
on the target class $t$ dimension:


\definecolor{azure}{rgb}{0.0, 0.5, 1.0}

\begin{equation}
	\begin{split}
    \frac{\partial \mathcal{L}_{\text{LOC}}}{\partial z^{t}_\mathcal{S}} &=  \frac{\partial \mathcal{L}_{\text{CE}}}{\partial z^{t}_\mathcal{S}} + \frac{\partial \mathcal{L}_{\text{KD}}}{\partial z^{t}_\mathcal{S}}  \\
    &=  \frac{\partial \mathcal{L}_{\text{CE}}}{\partial z^{t}_\mathcal{S}} + \frac{\partial{(\text{KL}(\mathbf{b}_{\mathcal{T}}||\mathbf{b}_{\mathcal{S}}) + p^{\backslash t}_{\mathcal{T}}  \text{KL}(\hat{\mathbf{p}}_{\mathcal{T}} || \hat{\mathbf{p}}_{\mathcal{S}}))}}{\partial z^{t}_\mathcal{S}}  \\
    &=  \frac{\partial \mathcal{L}_{\text{CE}}}{\partial z^{t}_\mathcal{S}} +
    \tcbhighmath{\frac{\partial {\text{KL}(\mathbf{b}_{\mathcal{T}}||\mathbf{b}_{\mathcal{S}})}}{\partial z^t_\mathcal{S}}} +
    \tcbhighmath[colback=green!8]{(p^{\backslash t}_{\mathcal{T}}) \times \frac{\partial \text{KL}(\hat{\mathbf{p}}_{\mathcal{T}} || \hat{\mathbf{p}}_{\mathcal{S}})}{\partial z^{t}_\mathcal{S}}}\\
    &= \underbrace{(p_\mathcal{S}^t - 1)}_{\in [-1,0]} + 
    \underbrace{\tcbhighmath{(p_\mathcal{S}^t - p_\mathcal{T}^{t})}}_{\in [-1,1]} + 
    \quad \tcbhighmath[colback=green!8]{0}.
    \label{eq:ce_grad}
    \end{split}
\end{equation}
Evidently, the gradient of $\text{KL}(\mathbf{b}_{\mathcal{T}}||\mathbf{b}_{\mathcal{S}})$ is uncontrollable and hinders the performance improvement. In particular,  when teacher model prediction on target class $t$ shows less confidence than student model, it poses contradictory objective with CrossEntropy. Hence, the student model struggles with the balance of under- and over-confidence problem. 

\noindent \textbf{Disentangle Knowledge Distillation}. In this work, we develop \FNTD{} (\FNTDab) that addresses both 1) and 2). we disentangle knowledge distillation to fully transfer inter  domain information and remove potential negative  performance impact. Thus, the \FNTD{} optimization objective for $i^{th}$ participant is: 

\begin{equation}
	\begin{split}
	   % \mathcal{L}_{\text{LOC}} &=\mathcal{L}_{\text{CE}} + \mathcal{L}_{\text{\FNTDab{}}}\\
    % &=
    % \mathcal{L}_{\text{CE}}+\cancelto{0}{\text{KL}(\mathbf{b}_{\mathcal{T}}||\mathbf{b}_{\mathcal{S}})} + \cancelto{1}{(1-p_{t}_{\mathcal{T}})} \ \text{KL}(\hat{\mathbf{p}}_{\mathcal{T}} || \hat{\mathbf{p}}_{\mathcal{S}}) \\
    % &= \mathcal{L}_{\text{CE}} + {\text{KL}(\hat{\mathbf{p}}_{\mathcal{T}} || \hat{\mathbf{p}}_{\mathcal{S}})}. \\
    % &=-\bm{1}_{Y_k}\log(\mathbf{p}(X_k,\theta_k))+\text{KL}(\hat{\mathbf{p}}(X_k,\theta_*) || \hat{\mathbf{p}}(X_k,\theta_k))
    \mathcal{L}_{\FNTDab{}} 
    &=
    \cancelto{0}{\text{KL}(\mathbf{b}_{\mathcal{T}}||\mathbf{b}_{\mathcal{S}})} + \cancelto{1}{(1-p^{t}_{\mathcal{T}})} \ \text{KL}(\hat{\mathbf{p}}_{\mathcal{T}} || \hat{\mathbf{p}}_{\mathcal{S}}) \\
    &= {\text{KL}(\hat{\mathbf{p}}_{\mathcal{T}} || \hat{\mathbf{p}}_{\mathcal{S}})}. \\
    &=\text{KL}(\hat{\mathbf{p}}(X_i,\theta_*) || \hat{\mathbf{p}}(X_i,\theta_i)),
    \label{eq:fntd}
    \end{split}
\end{equation}
where $\theta_*$ is the frozen model, which provides inter-domain knowledge. Besides, we maintain the CrossEntropy {\cite{CE_AOR05}} constraint to provide precise intra domain knowledge. Finally, the training target in local updating is:
\begin{equation}
    \mathcal{L}_{{LOC}} = \mathcal{L}_{{CE}} + \mathcal{L}_{\FNTDab{}}.
    \label{eq:localobj}
\end{equation}

\noindent \textbf{Comparison with \fccl{}}.
Leveraging previous model to regulate that the present model behavior should not deviate too much has also been considered in our conference paper, \fccl{} {\cite{FCCL_CVPR22}}. Specifically, \fccl{} conducts typical logits distillation in \cref{eq:kd_ork_form} with previous model and pretrained model, which is only trained on private data. However, directly aligning logits distribution consistency would affect the preserve of inter domain knowledge and interfere maintaining intra domain knowledge.


\subsection{Discussion}
We illustrate and summarize the proposed method in Figure 1 and \cref{alg:ours}. 
Our method can be viewed as how to learn more information from others in collaborative updating and how to maintain multiple domains knowledge in local updating. Firstly, we reach both logits-level and feature-level communication via  \FCCMab{} (\cref{sec:3.1})  and \FRSLab{} (\cref{sec:3.2}). Besides, it is applicable to large-scale scenario in federated learning, attributed to that the computation complexity is $\mathcal{O}(K)$. Notably, the operation of  \FCCMab{} and \FRSLab{} is respectively based on logits output and  similarity distribution regardless of the specific model structure. Thus, when participants share same model structure (model homogeneity),  ours is still capable. Secondly, in local updating, proposed \FNTDab{} (\cref{sec:3.3}) disentangles traditional logits knowledge distillation and focuses on transferring inter domain knowledge, which does not incur heavy computational overhead and not require complicated hyper-parameter setting.

\section{Experiments}
\noindent \textbf{Datasets and Networks}
We extensively evaluate our method on two classification tasks (\ie, \digits{} {\cite{MNIST_IEEE98,USPS_TPAMI94,svhn_NeurIPS11,syn_arXiv18}}, \officecaltech{} {\cite{OffCaltech_CVPR12}}, \officeTO {\cite{office31_ECCV10}} an \officehome {\cite{officehome_CVPR17}}) with two public data (\ie, \cifarhun{} {\cite{cifar_Toronto}}, \tyimagenet{} {\cite{ImageNet_IJCV15}} and \fashionmnist {\cite{fashionmnist_arXiv17}}). Specifically, \digits{} task includes four domains (\ie, \mnist{} ({M}), \usps{} ({U}), \svhn{} ({SV}) and \syn{} ({SY})) with $10$ categories. The \officehome{} task also have four domains (\ie, \art{} ({A}), \clipart{} ({C}),  \product{} ({P}) and \realworld{} ({R})). Note that for both tasks, data acquired from different domains present domain skew (\textbf{data heterogeneity}). 
For these four classification tasks, participants customize models that can be differ from differentiated backbones and classifiers (\textbf{model heterogeneity}). For experiments, we randomly set the model as \resnet \cite{ResNet_CVPR16}, \efficientnet {\cite{EfficientNet_ICML19}}, \mobilenet {\cite{Mobilenets_arXiv17}} and \googlenet {\cite{GoogLeNet_CVPR15}} for different domains.

\begin{figure}[t]
\centering
\subfigure[\digits{}]{
\includegraphics[width=0.47\linewidth]{Figure/Sample/Digists.pdf}
}
\subfigure[\officecaltech{}]{
\includegraphics[width=0.47\linewidth]{Figure/Sample/OfficeCaltech.pdf}
}
\subfigure[\officeTO{}]{
\includegraphics[width=0.47\linewidth]{Figure/Sample/Office31.pdf}
}
\subfigure[\officehome{}]{
\includegraphics[width=0.47\linewidth]{Figure/Sample/OfficeHome.pdf}
}


% \begin{subfigure}{0.24\linewidth}
% \includegraphics[width=\linewidth]{Figure/Example/example_art.pdf}
% \caption{\art{} (\textsl{A})}
% \end{subfigure}
% \begin{subfigure}{0.24\linewidth}
% \includegraphics[width=\linewidth]{Figure/Example/example_clipart.pdf}
% \caption{\clipart{} (\textsl{C})}
% \end{subfigure}
% \begin{subfigure}{0.24\linewidth}
% \includegraphics[width=\linewidth]{Figure/Example/example_product.pdf}
% \caption{\product{} (\textsl{P})}
% \end{subfigure}  
% \begin{subfigure}{0.24\linewidth}
% \includegraphics[width=\linewidth]{Figure/Example/example_realworld.pdf}
% \caption{\realworld{} (\textsl{R})}
% \end{subfigure}



\caption{\textbf{Example cases} in \digits{} {\cite{MNIST_IEEE98,USPS_TPAMI94,svhn_NeurIPS11,syn_arXiv18}}, \officecaltech{} {\cite{OffCaltech_CVPR12}}, \officeTO{} {\cite{office31_ECCV10}} and \officehome{} {\cite{officehome_CVPR17}} scenarios.}
\label{fig:example}
\end{figure}

\noindent \textbf{Metrics}
We report the standard metrics to measure the quality of methods: accuracy, which is defined as the number of samples that are paired divided by the number of samples. Specifically, for evaluation intra and inter domain performance, we define as following:

\begin{equation} \setlength\abovedisplayskip{1pt} \setlength\belowdisplayskip{1pt}
\mathcal{A}_i^{Intra}=\frac{\sum(\texttt{argMax}(f(\theta_i,X_i^{Test}))==Y_i^{Test})}{|D_i^{Test}|},
\label{eq:intraAcc}
\end{equation}

\begin{equation} \setlength\abovedisplayskip{2pt} \setlength\belowdisplayskip{1pt}
\mathcal{A}_i^{Inter}=\sum_{j \neq i}\frac{\sum(\texttt{argMax}(f(\theta_i,X_j^{Test}))==Y_j^{Test})}{(K-1)\times|D_j^{Test}|}.
\label{eq:interAcc}
\end{equation}

As for the method overall performance evaluation, we adopt the average accuracy as metric.
Besides, for these four classification tasks, \digits{}, \officecaltech{}, \officeTO{} and \officehome{} contain 10, 10, 31 and 65 categories. Top-1 and Top-5 accuracy are adopted for the first two and the latter two respectively.



\noindent \textbf{Counterparts}
We compare our proposed method against several state-of-the-art federated learning methods. 
First, for the model heterogeneity: \fedmd{} (NeurIPS' 19) {\cite{FedMD_NeurIPS19}}, \feddf{} \cite{FedDF_NeurIPS20} (NeurIPS' 20), \fccl{} \cite{FCCL_CVPR22} (CVPR' 22) and \rhfl{} \cite{RoFL_CVPR22} (CVPR' 22). Second, for the model homogeneity: \fedprox{} \cite{FedProx_arXiv2018} (arXiv' 18), \pfedme{} \cite{pFedME_NeurIPS20} (MeurIPS' 20), and \moon{} {\cite{MOON_CVPR21}} (CVPR' 21).

\noindent \textbf{Implement Details}
For a fail comparison, we follow {\cite{FedDF_NeurIPS20,MOON_CVPR21,FCCL_CVPR22,RoFL_CVPR22}}. Models are trained via Adam optimizer {\cite{Adam_arXiv14}} with batch size of $512$ and $256$ in collaborative updating and local updating. The learning rate is consistent $0.001$ in these two process for all approaches. We set the hyper-parameter  $\lambda=0.0051$ like {\cite{Barlow_ICML21}} and $\mu=0.02$ in {\cite{ISD_ICCV21}}). We further conduct hyper-parameter analysis of $\omega$ and $\tau$ in the following section.
As for data scale, in \digits{} task, the size of corresponding private data is set to $150$, $80$, $5000$ and $1800$ for \mnist, \usps, \svhn{} and \syn{}, respectively. 
As for \officehome{} task, each participant is individually assigned with \art, \clipart, \product{} and \realworld, and the corresponding private data size is $1400$, $2000$, $2500$, $2000$. We further list the private data scale for these four scenarios in the appendix.
The number of unlabeled public data is $5000$ for different scenarios. For pre-processing, we resize all input images into $32 \times 32$ with three channels for compatibility. We do communication  for $E=40$ epochs, where all approaches have little or no accuracy gain with more communications rounds. Besides, for \solo{}, models are trained on private data for $50$ epochs, which are also initial models for federated learning process.


\subsection{Comparison with SOTA Methods}
We comprehensively examine the proposed methods with state-of-the-art methods on four image classification tasks, \ie, \digits{} {\cite{MNIST_IEEE98,USPS_TPAMI94,svhn_NeurIPS11,syn_arXiv18}}, \officecaltech{} {\cite{OffCaltech_CVPR12}}, \officeTO{} {\cite{office31_ECCV10}} and \officehome{} {\cite{officehome_CVPR17}})) with two public data (\ie, \cifarhun{} \cite{cifar_Toronto} and \tyimagenet{} \cite{ImageNet_IJCV15}).

\noindent \textbf{Inter Domain Analysis.}  
We summarize the results of inter domain accuracy by the end of federated learning in \cref{table:interacc}. As shown in table, it clearly depicts that under domain shift, \solo{} present worst in these two tasks, demonstrating the benefits of federated learning. \oursabbv{} consistently outperforms all other counterparts on different scenarios. For example, in \digits{} scenario, \oursabbv{}  outperforms the best counterparts by  $29.32\%$ on \mnist{}, which means the average testing accuracy for respective model on \usps{}, \syn{} and \svhn{}.

\begin{table*}[t]\small
\centering
\caption{\textbf{Comparison of inter domain performance} with counterpart on the \cifarhun{}. \textbf{{M}$\to$} means that private data is \mnist{} and respective model is tested on other domains in \cref{eq:interAcc}. AVG denotes average accuracy calculated from each domain. (The best average accuracy is marked in bold. The best entries in each domain are underlined. These notes are the same to others.)}
\label{table:interacc}
{
\resizebox{0.90\textwidth}{!}{
\begin{tabular}{r||cccccIccccc}
\hline\thickhline
\rowcolor{mygray}
& \multicolumn{5}{cI}{\digits}&\multicolumn{5}{c}{\officecaltech}\\
\cline{2-11}
\rowcolor{mygray}
\multirow{-2}{*}{Methods}  &  {M}$\to$  & {U}$\to$  & {SV}$\to$  & {SY}$\to$  & AVG  & {AM}$\to$  & {CA}$\to$  & {D}$\to$  & {W}$\to$  & AVG \\

\hline\hline

\solo 
& 15.29 & 13.91 & 39.24 & 34.30 & 25.68 
& 28.20 & 32.11 & 19.99 & 28.11 & 27.10\\

\fedmd {\cite{FedMD_NeurIPS19}} 
&  8.97 & 12.61 & 40.89 & 43.03 & 26.38
& 19.14 & 31.24 & 17.48 & 25.09 & 23.23\\


\feddf {\cite{FedDF_NeurIPS20}} 
& 13.23 & 19.29 & 45.25 & 43.95 & 30.43
& 25.82 & 30.39 & 16.51 & 24.28 & 24.25\\
          
\fedmatch {\cite{FedMatch_ICLR21}} 
&  9.22 & 14.76 & 46.28 & 36.05 & 26.58  
& 19.25 & 32.21 & 13.80 & 22.66 & 21.98\\


\rhfl{} \cite{RoFL_CVPR22} 
& 19.15 & 16.72 & \underline{51.74} & 48.65 & 34.06
& 19.11 & 27.50 & 16.55 & 23.83 & 21.74   \\

\fccl{} \cite{FCCL_CVPR22} 
&{20.74} &  {20.60} &44.68& {48.02} & {33.51} 
& 25.16  & 33.68    &  17.52   & 23.81     & 25.04  \\
        
\oursabbv{} 
& \underline{34.15}  & \underline{48.95} & 51.29 & \underline{58.08} & \textbf{48.11}  
& 29.56  &  36.82  &  24.02  &    31.33   & 30.43 \\

\\

\hline\thickhline
\rowcolor{mygray}
& \multicolumn{5}{cI}{\officeTO}&\multicolumn{5}{c}{\officehome}\\
\cline{2-11}
\rowcolor{mygray}
\multirow{-2}{*}{Methods}  &  {AM}$\to$  & {D}$\to$  & {W}$\to$  &   & AVG  & {A}$\to$  & {C}$\to$  & {P}$\to$  & {R}$\to$  & AVG \\

\hline\hline

\solo 
& 21.08 & 27.93 & 34.14 & & 27.72   
& 18.89 & 19.36 & 21.97 & 21.02 & 20.31 \\

\fedmd {\cite{FedMD_NeurIPS19}} 
& 22.76 & 32.64   & 37.30 & &    30.90
& 16.85 &  23.13  &  28.78  &   25.01    & 23.44 \\

\feddf {\cite{FedDF_NeurIPS20}} 
& 24.74  & 26.7  & 35.4 &  & 28.96
& 17.38 &  21.76  &  25.17  &   22.97    & 21.82\\

\fedmatch {\cite{FedMatch_ICLR21}} 
& 22.23 & 31.98 & 40.15 &       & 31.45 
& 19.05 & 25.24 & 28.73 & 24.35 & 24.34 \\


\rhfl{} \cite{RoFL_CVPR22} 
& 20.52 & 20.59 & 36.32 & & 25.81
&   &     &     &      &   \\

\fccl{} \cite{FCCL_CVPR22} 
&24.89 &  30.73 &39.16 & & 31.59  
& {25.55} &  {26.41}  &  {30.14}  &   {29.41}    & {27.88} \\

\oursabbv{} 
& \underline{31.64} & \underline{36.94} & \underline{45.50} & & \textbf{38.02}  & 
& & \textbf{}\\
\end{tabular}}}

\end{table*}

\noindent \textbf{Intra Domain Analysis}
To compare the effectiveness of alleviating catastrophic forgetting on intra domain, we observe that our method almost outperforms the compared methods by a large margin along the federated learning process in \cref{fig:intrawithSOTA}. We further report the final intra domain accuracy in \cref{table:intraacc}.  \oursabbv{} suffers less periodic performance shock and is not prone to overfitting to local data distribution. The  \cref{table:interacc}  and \cref{table:intraacc} illustrate that \oursabbv{} is cable of balancing multiple domain knowledge and thus effectively alleviates catastrophic forgetting. 

\begin{table*}[t]\small
\centering
\caption{\textbf{Comparison of intra domain performance} with counterparts on the \cifarhun. The metric is evaluated on respective testing data in \cref{eq:intraAcc}.}
\label{table:intraacc}
{
\resizebox{0.90\textwidth}{!}{
\begin{tabular}{r||cccccIccccc}
\hline \thickhline
\rowcolor{mygray}
& \multicolumn{5}{cI}{\digits}&\multicolumn{5}{c}{\officecaltech}\\
\cline{2-11} 
\rowcolor{mygray}
\multirow{-2}{*}{Methods}  &  {M}  & {U}  & {SV}  & {SY}  & AVG  & {AM}  & {CA}  & {D}  & {W}  & AVG \\

\hline\hline

\solo 
& 70.20 & 74.19 & 74.57 & 73.60 & 73.14 
& 74.11 & 61.35 & 75.16 & 78.31 & 72.23\\

\fedmd {\cite{FedMD_NeurIPS19}} 
& 77.30 & 80.05 & 77.73 & 87.72 & 80.33
& 73.80 & 57.97 & 63.69 & 61.47 & 64.23\\

\feddf {\cite{FedDF_NeurIPS20}}  
& 82.95 & 78.84 & 78.46 & 91.30 & 83.38
& 71.16 & 57.73 & 67.94 & 71.08 & 66.97\\

\fedmatch {\cite{FedMatch_ICLR21}} 
& 82.69 & 78.31 & 79.79 & 89.23 & 82.69
& 73.38 & 60.25 & 68.58 & 73.56 & 68.94 \\

\rhfl{} \cite{RoFL_CVPR22} 
& 86.69 & 80.39 & \underline{88.44} & 97.90 & 88.35   
& 73.35 & 58.92 & 70.91 & 74.47 & 69.41  \\

\fccl{} \cite{FCCL_CVPR22} 
& 88.84 & 84.42 & 78.55 & 91.23 & 85.69
& 75.09 & 60.46 & 74.95 & 73.56 & 71.01 \\

\oursabbv{} 
& \underline{90.94} & \underline{88.52} & 86.83 & \underline{97.92} & \textbf{91.04}
& 75.26 & 59.90 & 75.80 & 75.48 & 71.60 \\

\\

\hline \thickhline
\rowcolor{mygray}
& \multicolumn{5}{cI}{\officeTO}&\multicolumn{5}{c}{\officehome}\\
\cline{2-11}
\rowcolor{mygray}
\multirow{-2}{*}{Methods}  &  {AM}  & {D}  & {W}  &   & AVG  & {A}  & {C} & {P}  & {R}  & AVG \\

\hline \hline

\solo 
& 72.95 & 77.31 & 80.88 & & 77.04    
& 65.27 & 60.50 & 74.68 & 54.28 & 63.68\\


\fedmd {\cite{FedMD_NeurIPS19}} 
& 70.36 & 73.89 & 78.58 & & 74.27 
& 66.17 & 60.63 & 76.35 & 56.60 & 64.93\\

\feddf {\cite{FedDF_NeurIPS20}} 
& 72.25 & 74.50 & 80.34 & & 75.69   
& 66.10 & 60.44 & 75.70  &   55.98 & 64.55\\

\fedmatch {\cite{FedMatch_ICLR21}} 
& 71.08 & 76.04 & 80.92 &  &  76.01   
& 81.50 & 65.40 & 79.81 & 65.06 & 72.94\\

\rhfl{} \cite{RoFL_CVPR22} 
& 70.98 & 73.90 & 78.87  & & 74.58 
&   &     &     &      &   \\


\fccl{} \cite{FCCL_CVPR22} 
&72.94 &  78.18 &81.72 & & 77.61 
& {81.51} &  65.42 &  {79.84}  &   {65.16} & 72.98\\

\oursabbv{} 
& 73.23  &  78.38  &  80.88   & & 77.49  & 
&  & \textbf{}\\

\end{tabular}}}
\end{table*}



% \oursabbv{} consistently outperforms all other counterparts on different datasets and memory buffer sizes. 

% We summarize the results of inter domain performance with counterparts in \cref{table:interacc}. It clearly depict that under domain shift, \solo{} present worst in these two tasks, demonstrating the benefits of federated learning.  We observe that \oursabbv{} significantly outperforms better than counterparts. As shown in table, \oursabbv{} consistently outperforms all other counterparts on different datasets and memory buffer sizes. 

% It shows strong robustness to many real-world challenges




\begin{figure*}[t]
\centering
\subfigure[\digits{}]{
\includegraphics[width=0.47\textwidth]{Figure/withSOTA/DigitsIntraWithSoTA.pdf}
}
\subfigure[\officecaltech{}]{
\includegraphics[width=0.47\textwidth]{Figure/withSOTA/CaltechIntraWithSoTA.pdf}
}
\caption{Comparison of average intra domain accuracy during federated learning process with sota methods on \cifarhun{}. We plot the \digits{} and \officecaltech{} scenarios. }
\label{fig:intrawithSOTA}
\end{figure*}

\subsection{Diagnostic Experiments}
For thoroughly assessing the efficacy of essential components of our approach, we perform an ablation study on \digits{} and \officeTO{}. to investigate the effect of each essential component: \FCCM{} (\FCCMab{} \cref{sec:3.1}), \FRSL{} (\FRSLab{} \cref{sec:3.2}) and \FNTD{} (\FNTDab{} \cref{sec:3.3}). We firstly give a  quantitative result of inter and intra domain performance on these three components in \cref{table:ablation}. The first row refers to a baseline that only respectively trains on private data.  The local updating phase for without \FNTD is remained same in our conference version, because \FCCMab{} and \FRSLab{} are designed for how to better learn from others in collaborative updating. Two crucial conclusions can be drawn. \textbf{First}, \FCCMab{} 


\begin{table*}[t]\small
\centering
\caption{\textbf{Ablation study of key components} in our proposed method. }
\label{table:ablation}
{
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{ccc||cccccIcccc}
\hline \thickhline
\rowcolor{mygray}
&&& \multicolumn{5}{cI}{\digits}&\multicolumn{4}{c}{\officecaltech}\\
\cline{4-12} 
\rowcolor{mygray}
\multirow{-2}{*}{\FCCMab{}}& \multirow{-2}{*}{\FRSLab{}} & \multirow{-2}{*}{\FNTDab{}} 
& M$\to$ & U$\to$ & SV$\to$ & SY$\to$ & AVG 
& AM$\to$ & D$\to$ & W$\to$ & AVG\\

\hline\hline

& & 
& 15.29 & 13.91 & 39.24 & 34.30 & 26.68
& 21.08 & 27.93 & 34.14 & 27.72\\

\ding{51}& & 
& 20.74 & 20.60 & 44.68 & 48.02 & 33.51
& 24.89 & 30.73 & 39.16 & 31.59\\

& \ding{51} & 
&&&&&
& 20.02 & 28.04 & 36.51 & 28.19  \\
       

\ding{51}& \ding{51}&
& 28.69 & 23.95 & 50.88 & 51.28  & 38.70
& 26.88 & 31.16 & 37.70 & 31.91\\

\ding{51}& \ding{51}& \ding{51}
& 34.15 & 48.95 & 51.29 & 58.08 & 48.11
& \textbf{31.64} & \textbf{36.94} & \textbf{45.50} & \textbf{38.02} \\
\\ 
\hline \thickhline
\rowcolor{mygray}
&&& \multicolumn{5}{cI}{\digits}&\multicolumn{4}{c}{\officecaltech}\\
\cline{4-12} 
\rowcolor{mygray}
\multirow{-2}{*}{\FCCMab{}}& \multirow{-2}{*}{\FRSLab{}} & \multirow{-2}{*}{\FNTDab{}} 
& M & U & SV & SY & AVG & {AM}  & {D}  & {W}  &    AVG   \\

\hline\hline

& & 
& 70.20 & 74.19 & 74.57 & 73.60 & 73.14 
& 72.95 & 77.31 & 80.88 & 77.04\\


\ding{51}& & 
& & & & & &
& & &\\

& \ding{51} & 
&   &   &   &   & 
&   &   &   & \\
\end{tabular}}}

\end{table*}

\begin{figure}[ht]
\begin{minipage}[]{0.56\linewidth}
\centering
% 	\setlength{\abovecaptionskip}{0.cm}
	\includegraphics[width=\linewidth]{Figure/FCCL/ab_fccl_inter.pdf}
\end{minipage}
\hfill
\begin{minipage}[]{0.42\linewidth}
\centering
\small{
\resizebox{\linewidth}{!}{
	\renewcommand\arraystretch{1.3}
	\begin{tabular}{r||c}
	\hline\thickhline
	\rowcolor{mygray}
	Public Data& AVG\\
    \hline\hline
    \cifarhun&33.51 \\
    \tyimagenet&35.70\\
    \fashionmnist& 36.82\\
	\end{tabular}
}}
\end{minipage}
\caption{\textbf{Ablation study on \FCCM{}} \cref{sec:3.1} \textbf{with different public data for inter domain performance} on each domain performance (left) and overall performance (right) in \digits{} task.}
\label{fig:ab_fcc_inter}
\end{figure}


\textbf{\FCCM{}}. 
To prove its robustness and stability, we evaluate the performance on different public data without label (\ie, \cifarhun{}, \tyimagenet{} and \fashionmnist{}). The results in \cref{fig:ab_fcc_inter} suggest that \FCCM{} achieves consistent performance in each domain. Moreover, it can be seen that it is more effective by the use of public data with rich categories (\tyimagenet) or simple detail (\fashionmnist). 
Besides, the \cref{fig:fcclHeatMap} presents that \FCCMab{}{} achieves similar logits output between participants and redundancy within the logits output, confirming that \FCCMab{} successfully enforces the correlation of same dimensions and decorrelation of different dimensions on both public and private data.



\begin{figure*}[t]
\centering

\subfigure[Epoch 1]{
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/1.pdf}
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/pri_1.pdf}
}
\put(-155,185){\textbf{\mnist}}
\put(-155,130){\textbf{\usps}}
\put(-155,75){\textbf{\svhn}}
\put(-155,20){\textbf{\syn}}
\subfigure[Epoch 2]{
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/2.pdf}
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/pri_2.pdf}
}
\subfigure[Epoch 5]{
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/5.pdf}
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/pri_5.pdf}
}
\subfigure[Epoch 10]{
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/10.pdf}
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/pri_10.pdf}
}
\subfigure[Epoch 15]{
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/15.pdf}
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/pri_15.pdf}
}
\subfigure[Epoch 20]{
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/20.pdf}
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/pri_20.pdf}

}
\subfigure[Epoch 30]{
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/30.pdf}
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/pri_30.pdf}

}
\subfigure[Epoch 40]{
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/40.pdf}
\includegraphics[width=0.1\textwidth]{Figure/FCCL/HeatMap/pri_40.pdf}
}
\put(-495,185){\textbf{\mnist}}
\put(-495,130){\textbf{\usps}}
\put(-495,75){\textbf{\svhn}}
\put(-495,20){\textbf{\syn{}}}


\caption{\small\textbf{ Cross-correlation matrix visualization} for different domains on \digits{} task with \cifarhun{}. The matrix is $10 \times 10$. We visualize the cross-correlation matrix (\cref{eq:avgcrosscorr}) with other models on public data (\textbf{Left Column}) during federated learning. Besides, for each domain, we represent the cross-correlation matrix with other models on  respective private data (\textbf{
Right Column}). The darker the color, the closer the $\mathcal{M}_i^{uv}$  is to $1$. See \cref{sec:3.1} for detail.}
\label{fig:fcclHeatMap}
\end{figure*}

\textbf{\FRSL}. We next examine the design of our \FRSL{}. As seen, the inter domain performance progressively improves as $\omega$ is increased, and the gain becomes relatively marginal when $\omega=2$ in different scenarios. Hence, we choose $\omega=2$  by default.

\begin{table}
	\centering
	\caption{\textbf{Analysis of $\omega$} for $\mathcal{L}_{\FRSLab{}}$ (Eq.~\ref{eq:col_loss}) on \digits{} and \officeTO{}.}
	\label{table:gammaabaltion}
	\small
	\resizebox{\columnwidth}{!}{
% 		\setlength\tabcolsep{5pt}
% 		\renewcommand\arraystretch{1.03}
		\begin{tabular}{c||ccccIccc}
			\hline\thickhline
			\rowcolor{mygray}
			$\omega$& \multicolumn{4}{cI}{\digits{}} & \multicolumn{3}{c}{\officeTO{}} \\ \cline{2-8}
			\rowcolor{mygray}
			Eq.~\ref{eq:col_loss} & M$\to$ & U$\to$ & SV$\to$ & SY$\to$ & AM$\to$ & D$\to$ & W$\to$ \\
			\hline\hline
			$1$ & 25.54 & 21.95 & 50.22 & 52.08
			    & 25.35 & \underline{31.22} & 37.57\\
			
			$2$ & \underline{28.69} & 23.95 & 50.88 & 51.28
			    & \underline{26.88} & \textbf{31.16} & \underline{37.70}\\

			$3$ & 30.97 & \textbf{25.90} & 51.12 & \underline{53.84}
			    & 24.88 & 30.54 & 36.53\\

			$4$ &  27.01 & \underline{24.12} & \textbf{52.08}  & 54.70
			    & \textbf{27.25} & 29.24 & \textbf{37.86}\\
		\end{tabular}
	}

\end{table}



\subsection{Hyper-Parameter Analysis}



